Mach cones in Heavy Ion Collisions

MACE, a model for the propagation of mach cones in the velocity field of heavy ion collisions (as created by hydrodynamical models) is explained. It is tested on an analytical test case (static medium) and applied to velocity fields created by the Particle-in-Cell model from LHC and RHIC initial conditions.

==> revision.tex <==
\vfill {\tiny Build 79; \today}

